Attacking the V: On the Resiliency of Adaptive-Horizon MPC

We introduce the concept of a V-formation game between a controller and an attacker, where controller's goal is to maneuver the plant (a simple model of flocking dynamics) into a V-formation, and the goal of the attacker is to prevent the controller from doing so. Controllers in V-formation games utilize a new formulation of model-predictive control we call Adaptive-Horizon MPC (AMPC), giving them extraordinary power: we prove that under certain controllability assumptions, an AMPC controller is able to attain V-formation with probability 1. We define several classes of attackers, including those that in one move can remove R birds from the flock, or introduce random displacement into flock dynamics. We consider both naive attackers, whose strategies are purely probabilistic, and AMPC-enabled attackers, putting them on par strategically with the controllers. While an AMPC-enabled controller is expected to win every game with probability 1, in practice, it is resource-constrained: its maximum prediction horizon and the maximum number of game execution steps are fixed. Under these conditions, an attacker has a much better chance of winning a V-formation game. Our extensive performance evaluation of V-formation games uses statistical model checking to estimate the probability an attacker can thwart the controller. Our results show that for the bird-removal game with R = 1, the controller almost always wins (restores the flock to a V-formation). For R = 2, the game outcome critically depends on which two birds are removed. For the displacement game, our results again demonstrate that an intelligent attacker, i.e. one that uses AMPC in this case, significantly outperforms its naive counterpart that randomly executes its attack.

==> algo_RPH.tex <==
% \SetAlgoSkip{}
%%%%% inner loop for finding next best action
\begin{algorithm}[b]
	\SetKwFunction{Fitness}{Fitness}
	\SetKwFunction{particleswarm}{particleswarm}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    
    $[\va^{h},\M^{h}] \leftarrow$ \particleswarm{$\mathcal{M},{p},h$}; \textit{// use 
    PSO in 
    order to determine best next action for the MDP $\mathcal{M}$ with horizon $h$\\}
    ${J}(s_{k+h})\leftarrow$ 
    \Fitness{$\M^h,\va^{h},{h}$};
    \textit{// calculate cost function if applying the first optimal action of horizon sequence of length $h$}\\
    \If{${J}(s_{k+h})\leqslant\widehat{J}$}
    {
   % $\Delta\leftarrow{J}(s_{i})/(m-i);$ \textit{// new level-threshold}\\
   		$\widehat{J}\leftarrow J(s_{k+h});$
        $\widehat{h}\leftarrow h;$ \textit{// store the horizon that has given the best cost so far}
    }
    
	\caption{RecedeHorizon ($\M,h,\widehat{J}$)}
	\label{alg:rhp}
\end{algorithm}
\setlength{\floatsep}{0.1cm}

==> birds_num.tex <==
\begin{tikzpicture}[scale=1, every node/.style={transform shape},auto, node distance=2cm,>=latex', cross/.style={path 
		picture={ 
			\draw[black]
			(path picture bounding box.south east) -- (path picture bounding 
			box.north west) (path picture bounding box.south west) -- (path picture 
			bounding box.north east);
		}}]
		
		%%%%%%%%%%%%%%%% blocks
		\tikzstyle{arrow} = [thick,draw=black,->,>=stealth]
		\tikzstyle{bird} = [circle, minimum width=.1cm, minimum 
		height=.1cm, draw=black, fill=yellow!20]
		\tikzstyle{output} = [coordinate]
		
		%%%%%%%%%%%% axis
		\draw[->] (0,0) -- (8,0) node[right] {$x$};
     	 	\draw[->] (0,0) -- (0,4.2) node[above] {$y$};
		
		%%%%%%%%%%%% birds
		\node (b1) [bird] at (1,1){$1$};
		\node (b2) [bird] at (2,1.5){$2$};
		\node (b3) [bird] at (3,2){$3$};
		\node (b4) [bird] at (4,2.5){$4$};
		\node (b5) [bird] at (5,2){$5$};
		\node (b6) [bird] at (6,1.5){$6$};
		\node (b7) [bird] at (7,1){$7$};
		
		%%%%%%%%%%%% velocities
		\draw[arrow] (b1) -- (1,2) {};
		\draw[arrow] (b2) -- (2,2.5) {};
		\draw[arrow] (b3) -- (3,3) {};
		\draw[arrow] (b4) -- (4,3.5) {};
		\draw[arrow] (b5) -- (5,3) {};
		\draw[arrow] (b6) -- (6,2.5) {};
		\draw[arrow] (b7) -- (7,2) {};

\end{tikzpicture}

==> diagram.tex <==
%%%%%%%%%%%%%%%%%%% colors
\definecolor{ShineSky}{rgb}{0, 0.9, 1}
\definecolor{ShineGrass}{rgb}{0.85, 0.88, 0.59}
\definecolor{InfosysDarkGrey}{gray}{0.4}
\definecolor{InfosysLightGrey}{gray}{0.6}
\definecolor{TuWienBlue}{cmyk}{1,0.38,0,0.15}
\definecolor{TuInfRed}{cmyk}{0,1,1,0}

%%%%%%%%%%%%%%%% blocks
\tikzstyle{block} = [draw, fill=ShineSky!20, rectangle, 
minimum height=3em, minimum width=6em]
\tikzstyle{conf} = [draw, fill=ShineSky!20, circle, node distance=0.7cm]
\tikzstyle{inv} = [draw, circle, node distance=0.7cm]
\tikzstyle{dots} = [->,>=stealth',shorten >=1pt,auto,node distance=2cm,
main node/.style={thick,circle,draw,font=\sffamily\Large}]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text 
centered, draw=black, fill=orange!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{pso} = [rectangle, rounded corners, minimum width=0.5cm, minimum 
height=0.5cm,text centered, draw=black, fill=gray!30]
\tikzstyle{fit} = [rectangle, rounded corners, minimum width=0.5cm, minimum 
height=0.5cm,text centered, draw=black, fill=gray!30]
\tikzstyle{box} = [fill=lightgray!45,rounded corners,minimum 
width=1.1cm,minimum height=4.02cm, anchor=north]
\tikzstyle{decision} = [diamond, aspect=1, minimum width=1cm, text 
centered, draw=black, fill=ShineGrass]
\tikzstyle{output} = [coordinate]

\begin{tikzpicture}[auto, node distance=2cm,>=latex', cross/.style={path 
	picture={ 
		\draw[black]
		(path picture bounding box.south east) -- (path picture bounding 
		box.north west) (path picture bounding box.south west) -- (path picture 
		bounding box.north east);
	}}]
	
	%%%%%%%%%%%%%% clones
	\node (start) [conf] {};
    \node [above = .2mm of start,text width=.3cm,align = center]{\scriptsize{$s_0$}};
	
% 	\node (c1) [conf, right = 5mm of start] {};
% 	\node (c2) [conf, above of=c1] {};
% 	\node (c3) [conf, above of=c2] {};
% 	\node (cn) [conf, below = 15mm of c1] {};
	
% 	\path (c1) -- node (dots) [auto=false]{\vdots} (cn);
	
% 	\draw [->] (start) -- (c1);
% 	\draw [->] ($ (start) !0.5! (c1) $) |- (c2);
% 	\draw [->] ($ (start) !0.5! (c1) $) |- (c3);
% 	\draw [->] ($ (start) !0.5! (c1) $) |- (c3);
% 	\draw [->] ($ (start) !0.5! (c1) $) |- (cn);
% 	\node [above = 0.2mm of c3,text width=2cm,align = 
% 	center]{\scriptsize{$s_0$}};
	
	%%%%%%%%%%%%% PSO	
	\node(pso1) [pso, right=3mm of start] {\scriptsize{PSO}};

	\draw [->] (start) -- (pso1);
	
	\node (c1n) [conf, right = 6mm of pso1] {};

	\draw [->] (pso1) -- node {\scriptsize{$\va^{h}$}} (c1n);
	
	%%%%%%%%%%%%%%%%%%%%% Fitness
	
	\node(fit1) [fit, right=6mm of c1n] {\scriptsize{${J}$}};

	\draw [->] (c1n) -- (fit1);
	
	%%%%%%%%%%%%%%%%%% Conditions
	\node (dec1) [decision, right = 1cm of fit1] {\scriptsize{$\ell_{i-1} - 
	\widehat{J} > \Delta_1$}}; 
	\draw[->] (fit1) -- node{\scriptsize{}}(dec1);
	\node (dec2) [decision,aspect=3, below = .5cm of dec1] {\scriptsize{${h} < 
	{h}_{max}$}};

	
    
    \node (step) [rectangle, text centered, draw=black, rounded corners, fill=gray!30, right = 7mm of dec1]{\scriptsize{Apply $a^1$}};
	
	\node (incH) [rectangle, text centered, draw=black, rounded corners, 
	fill=gray!30, left = 10mm of dec2]{\scriptsize{$h\mathrel{++}$}};
	
	\node (dec5) [decision,aspect=3, below = 4mm of dec2] {\scriptsize{${p} < 
	{p}_{max}$}};
	
	\node (incP) [rectangle, text centered, draw=black, text width=1.5cm, 
	rounded corners, fill=gray!30] at (incH |- dec5){\scriptsize{$h:=1;$}\\\scriptsize{$p\mathrel{+}=p_{inc};$}};
	
	\node (stuff) [rectangle, text centered, draw=black, rounded corners, 
	fill=gray!30, right = 12mm of step]{\scriptsize{$\ell_i:=\widehat{J}$}};
    
    \node (dec3) [decision,aspect=3, below = 4.1cm of stuff] 
	{\scriptsize{$\ell_i > \varphi$}};
    
    \node (dec4) [decision,aspect=3, below = 4mm of dec5] 
	{\scriptsize{$i < m$}};
    
    \node (incL) [rectangle, text centered, draw=black, rounded corners, 
	fill=gray!30] at (pso1 |- dec4){\scriptsize{$i\mathrel{++}$}};
  
	%%%%%%%%%%%%%% Arrows
	\draw[->](dec1.south) -- node(arr3){\scriptsize{No}} (dec2.north);
    
    \draw[->](dec1.east) -- node(arrApply){\scriptsize{Yes}}(step.west);
	
	\draw[->](stuff.south) |- (dec3.north);
    
	\draw[->](dec3.west) -- node(arr1)[above]{\scriptsize{Yes}} (dec4.east);
	\draw[->] (dec4.west) -- node(arr5)[above]{\scriptsize{Yes}} (incL.east);
	\draw[->] (incL.north) -- (pso1.south);
	\draw[->](dec2.west) -- node(arr6)[above,near start]{\scriptsize{Yes}} 
	(incH.east);
	\draw[->](incH.west) --  (incH -| incL);%(psoBox.south);
	
	\draw[->](step.east) -- (stuff);
	
	\draw[->](dec2.south) -- node[right]{\scriptsize{No}} (dec5.north);
	\draw[->] (dec5.west) -- node(arr7)[above,near 
	start]{\scriptsize{Yes}}(incP);
	\draw[->] (incP) -- (incP -| incL);%(psoBox.south);
	\node(V) [below = 4mm of dec3,text width=2cm,align = 
	center]{\scriptsize{\textbf{Stable state}}};
	\draw[->] (dec3.south) --node[right]{\scriptsize{No}} (V);
	\node(time) [below = 4mm of dec4,text width=2cm,align = 
	center]{\scriptsize{\textbf{Timeout}}};
	
	\draw[->] (dec4.south) --node[right]{\scriptsize{No}} (time);
	\node(exaust) [right = 6mm of dec5,text width=2.8cm,align = 
	center]{\scriptsize{\textbf{Particle exhaustion}}};
	\draw[->] (dec5.east) --node[above]{\scriptsize{No}} (exaust);
	
	\end{tikzpicture}

==> diagram2.tex <==
%%%%%%%%%%%%%%%%%%% colors
\definecolor{ShineSky}{rgb}{0, 0.9, 1}
\definecolor{ShineGrass}{rgb}{0.85, 0.88, 0.59}
\definecolor{InfosysDarkGrey}{gray}{0.4}
\definecolor{InfosysLightGrey}{gray}{0.6}
\definecolor{TuWienBlue}{cmyk}{1,0.38,0,0.15}
\definecolor{TuInfRed}{cmyk}{0,1,1,0}

%%%%%%%%%%%%%%%% blocks
\tikzstyle{conf} = [draw, fill=Yellow!20, circle, node distance=0.7cm]
\tikzstyle{inv} = [draw, circle, node distance=0.7cm]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{pso} = [rectangle, rounded corners, minimum width=0.5cm, minimum 
height=0.5cm,text centered, draw=black, fill=ShineSky!20]
\tikzstyle{fit} = [rectangle, rounded corners, minimum width=0.5cm, minimum 
height=0.5cm,text centered, draw=black, fill=ShineSky!20]
\tikzstyle{decision} = [diamond, aspect=1, minimum width=1cm, text 
centered, draw=black, fill=ShineSky!20]
\tikzstyle{output} = [coordinate]

\begin{tikzpicture}[auto, node distance=2cm,>=latex', cross/.style={path 
	picture={ 
		\draw[black]
		(path picture bounding box.south east) -- (path picture bounding 
		box.north west) (path picture bounding box.south west) -- (path picture 
		bounding box.north east);
	}}]
	
	%%%%%%%%%%%%%% configuration
	\node (start) [conf] {};
    \node [above = .2mm of start,text width=.3cm,align = center]{\scriptsize{$s_0$}};
	
	%%%%%%%%%%%%% PSO	
	\node(pso1) [pso, right=3mm of start] {\scriptsize{PSO}};

	\draw [->] (start) -- (pso1);
	
	\node (c1n) [conf, right = 6mm of pso1] {};

	\draw [->] (pso1) -- node {\scriptsize{$\va^{h}$}} (c1n);
	
	%%%%%%%%%%%%%%%%%%%%% Fitness
	
	\node(fit1) [fit, right=4mm of c1n] {\scriptsize{${J}$}};

	\draw [->] (c1n) -- (fit1);
	
	%%%%%%%%%%%%%%%%%% Conditions
	\node (dec1) [decision, right = 0.4cm of fit1] {\scriptsize{$\ell_{i-1} - 
	J > \Delta$}}; 
	\draw[->] (fit1) -- node{\scriptsize{}}(dec1);
    
    \node (fitCheck) [decision, aspect=3, below = 5mm of dec1]{\scriptsize{$J < \widehat{J}$}};
    
	\node (dec2) [decision,aspect=3, below = 5mm of fitCheck] {\scriptsize{${h} < 
	{h}_{max}$}};

% 	\node (applyMaxA) [rectangle, text centered, draw=black, rounded corners, fill=gray!50, below = 5mm of dec2] {\scriptsize{\textbf{Apply $a^h_1$}}};

 \node (setJh) [pso,text width=1cm, right =6mm of dec1]{\scriptsize{$\widehat{h}:=h$}\\\scriptsize{$\widehat{J}:=J$}};
    
    \node (step) [pso,right = 4mm of setJh]{\scriptsize{Apply $a^{\widehat{h}}_1$}};
	
	\node (incH) [pso,left = 10mm of dec2]{\scriptsize{$h\mathrel{++}$}};
	
% 	\node (dec5) [decision,aspect=3, below = 4mm of dec2] {\scriptsize{${p} < 
% 	{p}_{max}$}};
	
% 	\node (incP) [rectangle, text centered, draw=black, text width=1.5cm, 
% 	rounded corners, fill=gray!30] at (incH |- dec5){\scriptsize{$h:=1;$}\\\scriptsize{$p\mathrel{+}=p_{inc};$}};
	
 	\node (replace) [pso,text width=1cm] at (setJh |- fitCheck) {\scriptsize{$\widehat{J} \mathrel{:}= J$}\\\scriptsize{$\widehat{h} := h$}};
%     
	\node (incL) [coordinate,below = 4.5cm of pso1]{};
    
    
%     \node (dec4) [decision,aspect=3, below = 10mm of dec2] 
% 	{\scriptsize{$i < m$}};

%     \node (dec3) [decision,aspect=3] at (stuff |- dec4)
% 	{\scriptsize{$\ell_i > \varphi$}};

    \node (stuff) [pso,text width=1.2cm,align=left,right = 4mm of step] {\scriptsize{$\ell_i:=\widehat{J}$}\\\scriptsize{$i\mathrel{++}$}\\\scriptsize{$h:=1$}\\\scriptsize{$\widehat{J}:=inf$}};
    
    
    \node (setP) [pso, text width=1.5cm] at (incL |- replace){\scriptsize{$p\mathrel{:}=n \cdot h \cdot 2$}};

%     \node (resH) [rectangle, text centered, draw=black, rounded corners, 
% 	fill=gray!30, above = 3mm of incL]{\scriptsize{$h:=1$}};

	
  
	%%%%%%%%%%%%%% Arrows
	\draw[->](dec1.south) -- node(arr3){\scriptsize{No}} (fitCheck.north);
    \draw[->](fitCheck.south) -- node[right]{\scriptsize{No}}(dec2.north);
    \draw[->](dec1.east) -- node(arrApply){\scriptsize{Yes}}(setJh.west);
    \draw[->](setJh.east) -- (step);
	
	%\draw[->](stuff.south) -- (dec3.north);
    
	%\draw[->](dec3.west) -- node(arr1)[above]{\scriptsize{Yes}} (dec4.east);
	%\draw[->] (dec4.west) -- node(arr5)[above]{\scriptsize{Yes}} (incL.east);
% 	\draw[->] (incL.north) -- (resH.south);
%   \draw[->] (resH.north) -- (pso1.south);

	%\draw[->] (incL.north) -- (pso1.south);
    
    \draw[->] (incL.north) -- (setP.south);
    \draw[->] (setP.north) -- (pso1.south);
    
	%\draw[->](dec5.west) -- node(arr6)[above,near start]{\scriptsize{Yes}} 
	%(resH.east);
    \draw[->](dec2.west) -- node(arr6)[above,near start]{\scriptsize{Yes}} 
	(incH.east);
	\draw[->](incH.west) --  (incH -| incL);%(psoBox.south);
    %\draw[->](dec2.south) -- node[right]{\scriptsize{No}}(applyMaxA);
    
%     \draw[->](applyMaxA) -- (dec4);
	
	\draw[->](step.east) -- (stuff);
    \draw[->](fitCheck.east) -- node[above,near start]{\scriptsize{Yes}} (replace.west);
    \draw[->](replace.south) |- (dec2.east);

% 	\node(V) [below = 4mm of dec3,text width=2cm,align = 
% 	center]{\scriptsize{\textbf{Stable state}}};
% 	\draw[->] (dec3.south) --node[right]{\scriptsize{No}} (V);
% 	\node(time) [below = 4mm of dec4,text width=2cm,align = 
% 	center]{\scriptsize{\textbf{Timeout}}};
	
% 	\draw[->] (dec4.south) --node[right]{\scriptsize{No}} (time);

	\draw[-] (stuff.south) |- (incL.east);
	\draw[->] (dec2.south) --node[right]{\scriptsize{No}} ++(0,-.5) -|  (step.south);
	
	\end{tikzpicture}
